A Survey-Based Qualitative Study to Characterize Expectations of Software Developers from Five Stakeholders

Background: Studies on developer productivity and well-being find that the perceptions of productivity in a software team can be a socio-technical problem. Intuitively, problems and challenges can be better handled by managing expectations in software teams. Aim: Our goal is to understand whether the expectations of software developers vary towards diverse stakeholders in software teams. Method: We surveyed 181 professional software developers to understand their expectations from five different stakeholders: (1) organizations, (2) managers, (3) peers, (4) new hires, and (5) government and educational institutions. The five stakeholders are determined by conducting semi-formal interviews of software developers. We ask open-ended survey questions and analyze the responses using open coding. Results: We observed 18 multi-faceted expectations types. While some expectations are more specific to a stakeholder, other expectations are cross-cutting. For example, developers expect work-benefits from their organizations, but expect the adoption of standard software engineering (SE) practices from their organizations, peers, and new hires. Conclusion: Out of the 18 categories, three categories are related to career growth. This observation supports previous research that happiness cannot be assured by simply offering more money or a promotion. Among the most number of responses, we find expectations from educational institutions to offer relevant teaching and from governments to improve job stability, which indicate the increasingly important roles of these organizations to help software developers. This observation can be especially true during the COVID-19 pandemic.

==> Tables/key_findings.tex <==
\newcolumntype{v}{>{\hsize=.06\hsize}X}
\newcolumntype{k}{>{\hsize=.94\hsize}X}
% \newcolumntype{g}{>{\hsize=.3\hsize}X}
\newcolumntype{m}{>{\hsize=.2\hsize}X}

\begin{table*}[!ht]
    \centering
    \caption{Highlights of Findings from the Surveys}
    \begin{tabularx}{\textwidth}{v|k}
    \toprule
        \bf{RQ1} & \bf{Expectation from organization} \\ \midrule
        
        $1_{65}$ & What are your expectations from your organization? \newline
         \textbf{1) Learning Opportunities 7.32\%, 2) Goal Achievement 9.76\%, 3) Knack in Standard SE Practice 12.2\%, 4) Career Opportunities 21.95\%, 5) Work Benefits 29.27\%, 6) Proper Management 31.71\%, 7) Work-place Culture 48.78\%} \\ \midrule
         
         \bf{RQ2} & \bf{Expectation from manager} \\ \midrule
         
        $2_{105}$ & What are your expectations from your manager? \newline
        \textbf{1) Tech Savvy 13.33\%, 2) Career Opportunities 20.95\%, 3) Proper Management 43.81\%, 4) People Skill 48.57\%} \\ \midrule
        
        \bf{RQ3} & \bf{Expectation from peers} \\ \midrule
        
        $3_{85}$ & What are your expectations from peers in the team? \newline
        \textbf{1) Learning Environment 10.59\%, 2) Sincerity 43.53\%, 3) Knack in Standard SE Practice 54.12\%, 4) Supportive Attitude 55.29\%} \\ \midrule
        
        \bf{RQ4} & \bf{Expectation from the new hires} \\ \midrule
        
        $4_{34}$ & What are your expectations from the new hires? \newline
        \textbf{1) Knack in Standard SE Practice 47.06\%, 2) Sincerity 47.06\%, 3) Motivation for Learning 52.94\%} \\ \midrule
        
        \bf{RQ5} & \bf{Expectation from the universities and the government} \\ \midrule
        
        $5_{70}$ & What are your expectations from the universities? \newline
        \textbf{1) Learning Environment 21.43\%, 2) Career Support 27.14\%, 3) Industry Oriented Teaching 77.14\%} \\ \midrule
        
        $6_{65}$ & What are your expectations from the government? \newline
        \textbf{1) Proper Education 23.08\%, 2) Career Opportunities 24.62\%, 3) Support for Industry 29.23\%, 4) Policy and Facility 63.08\%} \\
        
    \bottomrule
    \end{tabularx}
Subscript with a question number shows number of responses
    \label{table:key_findings}
\end{table*}

==> Tables/participants_role.tex <==
\begin{table}[b]
\centering
\caption{Role wise Distribution of Participants}
\begin{tabular}{|c|c|}
\hline
\textbf{Role of the Participants} & \textbf{Percentage}\\
\hline
Developer & 69.72\%\\
Manager & 16.9\%\\ 
SQA Engineer & 7.04\%\\
Business Analyst & 1.4\%\\
R\&D Engineer & 1.4\%\\
Data Engineer & 0.7\%\\
Software Architect & 0.7\%\\
Team Lead & 0.7\%\\
Trainer & 0.7\%\\
UX Designer & 0.7\%\\
\hline
\end{tabular}
\label{tab:role}
\end{table}
